I3DE: An IDE for Inspecting Inconsistencies in PL/SQL Code

In this paper, we introduce I3DE (Inconsistency Inspecting IDE) - an IDE plugin to inspect inconsistencies in PL/SQL code. We first observed the potential issues, e.g., misuses or bugs, that are introduced by the inconsistent understanding of PL/SQL semantics by PL/SQL programmers and DBMS developers, and propose a metamorphic testing-based approach for inspecting such inconsistencies in PL/SQL code. We design and implement our approach in I3DE, a widely usable plugin for the IntelliJ Platform. We conducted a comparative user study involving 16 participants, and the findings indicate that I3DE is consistently effective and efficient in helping programmers identify and avoid inconsistencies across different programming difficulties

==> sections/2_PLSQL_IC3_Figure_Translation.tex <==
\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\textwidth]{figs/fig_translate_1.png}
    \caption{translate assignment statement in PL/SQL to plain SQL}
    \label{fig:sub1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\textwidth]{figs/fig_translate_2.png}
    \caption{translate conditional control statement in PL/SQL to plain SQL}
    \label{fig:sub2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\textwidth]{figs/fig_translate_3.png}
    \caption{translate iterative statement in PL/SQL to plain SQL}
    \label{fig:sub3}
  \end{subfigure}
  \caption{Translate PL/SQL statements to plain SQL. \ls{Do we need both of them?}}
  \label{fig:translation_example}
\end{figure}


==> sections/3_IDE_Integration_Figure_Categories.tex <==
\begin{figure}[t]
\centerline{\includegraphics[width=0.9\linewidth]{figs/fig-inconsistency-categorie.png}}
\caption{Architecture of PL/pgSQL Engine}
\label{fig:arch-plpgsql}
\end{figure}
